Compiler generated feedback for Large Language Models

We introduce a novel paradigm in compiler optimization powered by Large Language Models with compiler feedback to optimize the code size of LLVM assembly. The model takes unoptimized LLVM IR as input and produces optimized IR, the best optimization passes, and instruction counts of both unoptimized and optimized IRs. Then we compile the input with generated optimization passes and evaluate if the predicted instruction count is correct, generated IR is compilable, and corresponds to compiled code. We provide this feedback back to LLM and give it another chance to optimize code. This approach adds an extra 0.53% improvement over -Oz to the original model. Even though, adding more information with feedback seems intuitive, simple sampling techniques achieve much higher performance given 10 or more samples.

==> tables/test-data.tex <==
\begin{table}
  \caption{%
    Test data.
  }
  \label{tables/test-data}
  \centering
  \begin{tabular}{lC{1.25cm}C{1.75cm}C{1.6cm}}
    \toprule
    & $n$ functions & unoptimized instruction count & -Oz instruction count \\
    \midrule
    AI-SOCO~\cite{ai-soco} & 8,929 & 97,800 & 47,578 \\
    ExeBench~\cite{exebench} & 26,806 & 386,878 & 181,277 \\
    POJ-104~\cite{poj104} & 310 & 8,912 & 4,492 \\
    Transcoder~\cite{transcoder-ir} & 17,392 & 289,689 & 129,611 \\
    % \midrule
    CSmith~\cite{csmith} & 33,794 & 647,815 & 138,276 \\
    YARPGen~\cite{yarpgen} & 12,769 & 285,360 & 144,539 \\
    \midrule
    Total & 100,000 & 1,716,354 & 645,773 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/training-data.tex <==
% \begin{table}
%   \caption{%
%     Training data. Each LLVM-IR function is autotuned and used to create a (Prompt, Answer) pair. The $n$ tokens column shows the number of tokens when the prompt is encoded using the Llama 2~\cite{llama} tokenizer.
% }
%   \label{tables/training-data}
%   \centering
%   \begin{tabular}{lC{1.13cm}C{1.5cm}C{1.2cm}c}
%     \toprule
%     & $n$ functions & unoptimized instruction count & size on disk & $n$ tokens \\
%     \midrule
%     Handwritten & 610,610 & 8,417,799 & 653.5 MB & 214,746,711 \\
%     Synthetic & 389,390 & 13,775,149 & 352.3 MB & 158,435,151 \\
%     \midrule
%     Total & 1,000,000 & 16,411,249 & 1.0 GB & 373,181,862 \\
%     \bottomrule
%   \end{tabular}
% \end{table}
% 


\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{img/llm_data.png}}
\caption{%
    Training and test data. Each LLVM-IR function is autotuned and used to create a (Prompt, Answer) pair. The $n$ tokens column shows the number of tokens when the prompt is encoded using the Llama 2~\cite{llama} tokenizer.
}
\label{tables/llm_data}
\end{center}
\end{figure}

